Fast Imbalanced Classification of Healthcare Data with Missing Values

In medical domain, data features often contain missing values. This can create serious bias in the predictive modeling. Typical standard data mining methods often produce poor performance measures. In this paper, we propose a new method to simultaneously classify large datasets and reduce the effects of missing values. The proposed method is based on a multilevel framework of the cost-sensitive SVM and the expected maximization imputation method for missing values, which relies on iterated regression analyses. We compare classification results of multilevel SVM-based algorithms on public benchmark datasets with imbalanced classes and missing values as well as real data in health applications, and show that our multilevel SVM-based method produces fast, and more accurate and robust classification results.

==> Algorithms.tex <==
%%\section{Supervised Classification Algorithms for Medical Data}
%
%Supervised classification methods aim to build an optimal classifier based on training data with known class labels and predict the label of test data. A classification problem is known as imbalanced classification, while the size of classes are not equal. Most classification problems in healthcare field are imbalanced in practice. Examples of such problems can be found in disease diagnosis \cite{khalilia2011predicting}, DNA microarray data classification \cite{yu2013acosampling}, the discharge status prediction at intensive care unit (ICU) \cite{roumani2013classifying}, and risk prediction for hospital readmission \cite{zolfaghar2013predicting}. Typically the classical classification algorithms do not perform well for these problems because they tend to train models with respect to the majority class and pay less attention to the minority class ( or so-called positive class). 
%
%Cost-sensitive learning is one the most common method to handle the imbalanced classification problems. This method penalizes the minority class misclassification through cost coefficient, which are inversely proportional to the size of each class. The cost-sensitive extension of support vector machine (SVM) is known as the wighted support vector machine (WSVM) \cite{lin2002fuzzy}.   
%
%In addition to imbalanced nature of  data in health applications, there are two main concerns: 
%\begin{itemize}
%  \item Medical data often exposed to missing features and can highly deteriorate the efficiency of most machine learning 
%  \item The size of data is often large due to increasing medical records, therefore regular SVM and WSVM is inappropriate and very time-consuming
%\end{itemize}
%
%%Another issue about imbalanced classification is the presence of missing feature data.
%In practice, real data, particularly in healthcare, often suffer from missing values or incomplete features. Missing values occur for various reasons. Certain medical tests cannot be repeated due to lack of the required medical equipments or their risks for certain patients; medical records might be corrupted due to malfunctions or error by human or equipments. Sometimes, certain medical tests takes longer and it might be necessary to make a preliminary decision about a disease based on the current test results that is available. These circumstances can increasingly create bias in the classification and predictive modeling and can lead to wrong decisions \cite{nanni2012classifier}. The performance of prediction model is highly correlated to the rate of missing values. 
%The literature on missing values in data has been well studied in the classical statistical analysis field \cite{ghannad2010selection,little2002statistical,schafer2010analysis}, but less studied in the machine learning domain. In recent years, this filed of research has attracted a lot of attention \cite{garcia2010pattern,gheyas2010neural}. 
%
%
%% Missing feature imputation methods are one of the most popular way to deal with this problem.
%Problems with missing data can be categorized into three types: data is completely at random (MCAR), missing at random (MAR), and not missing at random (NMAR). MCAR occurs while any feature of a data instance is missing completely random and is independent of the values of other features. Data is MAR , when the data instance with missing feature is dependent on the value of one or more of the instances’ other features. NMAR occurs when the data instance with missing feature is dependent on the value of the other missing features. Even though MCAR is more desirable, in many real-world problems, MAR occurs frequently in practice \cite{ghannad2010selection}. Typically most approaches for imbalanced classification demonstrate poor performance in an environment with missing values and this leads into wrong decisions in medical domain. Previous work has shown that use of SVM-based algorithms becomes problematic in the presence of missing features \cite{farhangfar2008impact} and yield poor performance. 
%On the other hand, using nonlinear SVMs is often time consuming and needs more computational resources as the size data becomes extremely large. Hence we aim to develop methods that take into consideration the specific character of large and imbalanced
%data classification, and on the other hand, they are robust with respect to missing values.
%
%A simple approach to deal with this problem is to ignore the data points that contain missing features and builds the classifier based on the complete data features \cite{rubin1976inference,jerez2010missing,garcia2010pattern}. This technique, commonly known as filtering, is applicable in practice, but it can be problematic in the presence of high percentage of missing features and may cause serious bias in data analysis and classification. For example in biology, ignoring the genes that consist of missing features is impractical since a large extent of data in the matrix could be discarded \cite{pan2011towards}. Another approach to deal with missing values is the so-called imputation. Missing-data imputation method substitutes a missing value with a meaningful estimation \cite{garcia2010pattern}. These methods estimate missing values either directly from the information in the dataset or by constructing a predictive model to do this purpose. Typical methods for imputation are mean imputation \cite{donders2006review}, kNN imputation \cite{batista2002study}, Bayesian principal component analysis (BPCA) imputation \cite{oba2003bayesian}, and the expectation maximization (EM) \cite{schneider2001analysis}. 
%
%EM is a more sophisticated and powerful method \cite{huang2009maximum}. This method is an iteratively applies linear regression analyses and fits a new linear to the estimated data until a local optimum is achieved \cite{ghahramani1994supervised,schneider2001analysis}.  In the regularized adaption of EM method, the conditional maximum likelihood estimation of regression parameters is replaced in the conventional EM algorithm \cite{nanni2012classifier}. 
%
%The SVM-based classification algorithms become intractable and computationally expensive when the size of data is very large. 
%In this paper, we develop a new method for more robust and effective solution of SVM and WSVM. The main intuition lies on a multilevel algorithmic framework (MF) originated from the multiscale optimization strategies \cite{brandt:optstrat}. At the original level, data are sorted from no missing feature to the highest number of missing features. In fact, it tends to choose data with maximum number of known features and give less priority to uncertain data in the training process. This hierarchal algorithm reduces the effect of missing value at each level and obtain a robust optimal classifier on large-scale data.  It also yields a linear complexity,
%and easily adjusted to parallelization. The MF framework has been very effective in many practical machine learning tasks including clustering \cite{mlmodul,KushnirGB06}, segmentation \cite{sharon06Hierarchy}, and dimensionality reduction \cite{raey}.
%
%The contribution of this paper is a new classification multilevel algorithmic approach for missing feature problem using scalable SVM and WSVM and EM methods. In this paper, we propose a multilevel algorithm that first builds priority on data with missing features in the training set and then produces a hierarchy of coarse subsets of the original large-scale training set, obtains SVM (or WSVM) classifier at the coarsest level with fewer data points, and updates the optimal classifier gradually though refinement of the support vectors. We compare classification results from multilevel SVM and WSVM to those from standard SVM, WSVM, logistic regression, Naive Bayes, tree learning on public benchmark datasets in UCI machine learning repository \cite{UCI}. We demonstrate that the proposed method produces superior results on both balanced and imbalanced datasets with missing features. This method requires considerably less memory compared to regular SVMs. 


==> Medicalintro.tex <==
\section{The role of predictive modeling in healthcare}
Modern healthcare can be characterized as \textit{evidence-driven} and \textit{model-assisted} \cite{foldy2014national}. In an ideal situation, every decision in the clinical environment should be supported by a statistical predictive model for risks and possible outcomes. This model may have a form of a simplified risk-assessment formula \cite{haas2013risk}, or a sophisticated machine learning tool \cite{plis2014machine}, \cite{woolery1994machine}. In either case, the model is based on a query from a database containing relevant examples from medical and operational history. 

In practice, comprehensive medical information is stored in  separate databases, with different formats and rules of access. Due to considerations of patient privacy, and the proprietary nature of electronic medical records \cite{larson2004survey}, the databases cannot be queried continuously. Every instance of data acquisition and integration is a separate effort that is cost-effective only when the resulting predictive model shows very high quality. Thus, progress in evidence-driven healthcare depends on how well state-of-the art algorithms of machine learning are adapted to clinical data.

We note that classical computer science issues, such as scalability, or convergence rate are rarely an issue in machine learning for healthcare. Instead, an algorithm is ranked based on its ability to process raw medical data, with such problematic features as sparsity (including accidentally missing data) and imbalanced outputs. Massive medical data is inherently sparse because of the encounter nature of patient-hospital interaction. When a clinical encounter occurs, some labels are attached to it \cite{snomed2011systematized}; the number and contents of labels vary widely, and at all other times the state of the patient is unknown. The outcomes of interest in classification problems are inherently imbalanced because, as a rule, healthcare analytics is motivated by data with evidence of crisis, severe health conditions, gaps and bottlenecks in access to care, all of these are rare events.

Many of such issues are not obvious from the perspective of a local healthcare provider (such as a single doctor); by definition they have access to all knowledge they ever use. We view this paper as a short, high-level primer on using advanced methods of machine learning to overcome the difficulties that emerge after multiple datasets are integrated for analysis and prediction.

This work was prompted by several projects completed with the Division of Applied Research and Clinical Informatics, Dept. of Data Science; Geisinger Health System. The routine activity of Data Science consists of medium-scope predictive projects on a combination of patient biometrics, pathology lab results, clinical encounter data, medical insurance data (available directly from Geisinger Health Plan) and externally assigned aggregate metrics for patients' general lifestyle risks, compliance with treatment regime, and loyalty to a particular provider. 

For the first motivating example, we use our 2014 feasibility study \cite{RoderickMEDAI} of merging insurance information (6 aggregate features, based on the history of claims and payments) together with clinical encounter information (10-20 features chosen by hand from patient biometrics, medications and diagnostic codes). The goal of the initial study was to predict the financial risk for a particular patient (a common metric in insurance practice, derived as a ratio of individual expenses and average expenses for a large demographic group). Furthermore, we wanted to see how addition of the clinical information changes the predictive power of the model, thus making a case for existence of high-risk patients that are invisible to claims-based analysis. We used a standard clustering technique, k-nearest neighbors with empirically selected weighting, to achieve the basic results.

For the second example, we use our preliminary investigation of patients' response to public outreach \cite{RoderickFLU}, such as annual flu awareness campaigns. We included basic demographic and clinical information on patients targeted by 35 such campaigns into the model predicting whether a given patient is likely to respond to the reminder, or to choose not to get vaccinated, or use a different provider. Again, our core predictive model was standard: logistic regression with empirically selected weighting of training data.

We now pose a question: how much more effective would the predictive models be in each case with the use of an advanced machine learning algorithm developed with awareness of sparsity and class skewness (imbalance) in data?

\section*{Additional notes}

Note: use this for the numerical results section.

The first table is based on Example 1, a classification task of placing a patient in a correct group by financial risk (ordered from 1 to 5). The motivation of the original study was to determine how much integration of the medical and financial data changes the outcomes of clustering and classification operations based on financial data alone. For that purpose, modest precision was sufficient; we used a logistic (linear) regression approach (implemented as \textit{mnrfit} in Matlab). We are comparing the precision of with the best results obtained by multilevel support vector machine method.

\begin{tabular}{|c|c|c|c|c|c|}
	\hline Class of financial risk & 1 & 2 & 3 & 4 & 5 \\ 
	\hline Precision using logistic regression & 0.58 & 0.54 & 0.53 & 0.51 & 0.59 \\ 
	\hline Precision using SVM & 0.73 & 0.50 & 0.44 & 0.50 & 0.71 \\ 
	\hline 
\end{tabular} 

To interpret the results, please note that correct identification of intermediate risk categories is a very difficult problem in medical informatics. To our knowledge, there is no good definition of "average health", either evidence-driven or philosophical, that would help an expert to identify such patient features that do not indicate an acute crisis, or an almost certain safety from crisis. Accordingly, it is not surprising that neither approach does well on the risk categories 2..4; there is also not a lot of motivation to improve the model there.
On the other hand, it is important to identify and predict the very low-risk patients (knowing that status ahead of time allows resource re-allocation leading to savings and improved service for everyone) and the very high-risk patients (so that clinical and financial resources could be prepared for the forthcoming crisis).

Accordingly, it is important that the use of an advanced method of machine learning changes the quality of prediction from almost worthless ('toss a coin') to workable (precision of $0.7$). 

In the second table, we are comparing results for the basic approach and a support vector machine prediction for Example 2, a study of patient's response to hospital flu outreach. This example involves a binary classifier: either the patient will get vaccinated after reminder, or not (this includes using a different provider) In the preliminary study, we used adaptive linear regression model (LASSO for adaptive selection of features, logistic regression on actual prediction). We compare with two versions of SVM.

\begin{tabular}{|l|l|l|l|}
	\hline  & Sensitivity  & Specificity & Accuracy \\ 
	\hline Adaptive logistic regression & 0.8903 & 0.6345 & 0.7619 \\ 
	\hline Standard SVM & 0.9750 & 0.6583 & 0.8496 \\ 
	\hline Weighted SVM & 0.9739 & 0.6598 & 0.8495 \\ 
	\hline 
\end{tabular} 

Response to outreach is not a crucial life-or-death issue, we are performing this study to see if predictive modeling can assist with resource allocation (which patients to contact, how much medical personnel effort to dedicate to outreach and then vaccination). Arguably, accuracy is more important than specificity here. 
Even the basic results (using linear regression) were met with approval the CPSL (Care Patient Service Line: a division responsible for coordinating efforts of local, small-scale healthcare providers operating under Geisinger). SVM methods (almost 10 percent improvement) provide additional justification for the use of machine learning on merged data to assist planning in clinical practice.


==> README <==
January 10, 2007

Please note that you may choose to use either double column or single column
formatting. You may wish to use single column formatting when submitting your
paper for review, as it leaves more space for reviewer remarks. The double column format 
is ideal when submitting your final publication materials. The IEEE CS formats articles
in two columns, with 9.5pt Palatino font, and a page size of 7.875 X 10.75. 

June 6, 2006

Added an option to switch between peer review and final submission formats 
into bare_jrnl.tex. 


August 13, 2002

This IEEEtran.cls is the official LaTeX class for authors of the
Institute of Electrical and Electronics Engineers (IEEE) transactions
journals and conferences. In addition to being carried on IEEE's site,
IEEEtran.cls may be found at:

http://www.ctan.org/tex-archive/macros/latex/contrib/supported/IEEEtran/

The CTAN site may have additional files related to non-IEEE uses of this
tool.

As of version 1.6, IEEEtran.cls now provides support for conferences and
A4 paper. Users of previous versions should no longer manually alter margins,
paper sizes, page styles, etc. Also, please note that \author is used
slightly differently from that of V1.5, especially for conferences.
\pubid (if used) must now be placed before \maketitle. \cite is now robust
and can be used within captions without a proceeding \protect.

As with previous versions, The itemize, enumerate, and description lists as
well as \appendix(ces) have enhanced controls and work slightly differently
than is done in traditional LaTeX.

Extensive formal documentation is now available. Enjoy! ;) The appendices
of the user manual contain important information on avoiding commonly
made mistakes, compatibility issues and installation instructions.


Best wishes for all your publication endeavors,

Michael Shell
mshell@ece.gatech.edu



********************* Files **********************

README               - This file.

IEEEtran.cls         - The LaTeX class file.

IEEEtran_HOWTO.pdf   - The user manual.

bare_jrnl.tex        - A "bare bones" starter file for journal papers.




**********************************************************************
 Legal Notice:
 This code and advice is offered as-is without any warranty either
 expressed or implied; without even the implied warranty of
 MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE!
 User assumes all risk.
 In no event shall IEEE or any contributor to this code
 be liable for any damages or losses, including, but not limited to,
 incidental, consequential, or any other damages, resulting from the
 use or misuse of any information contained here.
 
 All statements made here are the opinions of their respective
 authors and are not necessarily endorsed by the IEEE.

 This code/text is distributed under the Perl Artistic License 
 ( http://language.perl.com/misc/Artistic.html ) 
 and may be freely used, distributed and modified.
 Retain all contribution notices and credits.
**********************************************************************




==> alg.tex <==
\section{Method}







==> alg_Refine.tex <==
\subsection{The Refinement Phase}
\label{refine}


==> discussion.tex <==
\section{Discussion}\label{sec:disc}


==> future.tex <==
\paragraph{Future research and possible improvements.}


